Pushdown Control-Flow Analysis for Free

Traditional control-flow analysis (CFA) for higher-order languages, whether implemented by constraint-solving or abstract interpretation, introduces spurious connections between callers and callees. Two distinct invocations of a function will necessarily pollute one another's return-flow. Recently, three distinct approaches have been published which provide perfect call-stack precision in a computable manner: CFA2, PDCFA, and AAC. Unfortunately, CFA2 and PDCFA are difficult to implement and require significant engineering effort. Furthermore, all three are computationally expensive; for a monovariant analysis, CFA2 is in $O(2^n)$, PDCFA is in $O(n^6)$, and AAC is in $O(n^9 log n)$. In this paper, we describe a new technique that builds on these but is both straightforward to implement and computationally inexpensive. The crucial insight is an unusual state-dependent allocation strategy for the addresses of continuation. Our technique imposes only a constant-factor overhead on the underlying analysis and, with monovariance, costs only O(n3) in the worst case. This paper presents the intuitions behind this development, a proof of the precision of this analysis, and benchmarks demonstrating its efficacy.

==> SecBisimulation.tex <==


\section{Proof of Precision}
\label{sec:proof}
%
To illustrate more formally how our optimization yields a finite-state abstraction with equivalent precision to PDCFA and AAC, we define 
a simulation relation $(\simXi)$ where $\hat{\xi} \simXi \tilde{\xi}$ (read as ``$\hat{\xi}$ simulates $\tilde{\xi}$'') if and only if all stored values and machine configurations in $\tilde{\xi}$  
(including stacks implicit in this configuration) are accounted for in the unbounded-stack representation $\hat{\xi}$.
%
The reader should also recall our discussion of soundness in section~\ref{sec:background:soundness} as this represents the other half $(\sqsubseteq)$ of what is 
more fully a bidirectional isomorphism between these machines.
%
In this section we focus exclusively on the portion of this isomorphism that is novel in our work: precision.
%
We begin by defining the simulation relation between the corresponding parts of the machines:
%
\begin{align*}
  (\simXi) &\subseteq \hat{\Xi} \times \tilde{\Xi}  && \text{[state-space simulation]}
  \\
  (\simX) &\subseteq \hat{\Xi} \times \tilde{\Sigma} && \text{[partition simulation]}
  \\
  (\simEnv) &\subseteq \widehat{Env} \times \widetilde{Env}  && \text{[env. simulation]}
  \\
  (\simStore) &\subseteq \widehat{Store} \times \widetilde{Store}  && \text{[store simulation]}
  \\
  (\simD) &\subseteq \hat{D} \times \tilde{D}  && \text{[flow-set simulation]}
  \\
  (\simClo) &\subseteq \widehat{Clo} \times \widetilde{Clo}  && \text{[closure simulation]}
  \\
  (\simKont) &\subseteq \hat{K} \times \widetilde{Addr} \times \widetilde{KStore}  && \text{[kont simulation]}
\end{align*}
%
We will use $\hat{k} \in \hat{K} = \PowSm{\widehat{Kont}}$ to denote sets of unbounded-stacks. 
%
This domain simulates $\tilde{K}$ in the finite-state machine.
%
Our ternary $(\simKont)$ relation will be styled like so:
%
\begin{align*}
  (\hat{k}, \tilde{a}_\cont, \tilde{\sigma}_\cont) \in (\simKont) 
  \iff
  \hat{k} \simR \tilde{a}_\cont \text{  (via $\tilde{\sigma}_\cont$)}
\end{align*}
%
Environments, value-stores, flow-sets, and closures simulate under the straightforward structural liftings we would expect given their identical layout.
%
\begin{align*}
  \hat{\rho} \simEnv \tilde{\rho} &\iff \forall \vv \in dom(\tilde{\rho}).\ \hat{\rho}(\vv) \simAddr \tilde{\rho}(\vv) 
  \\
  \hat{\sigma} \simStore \tilde{\sigma} &\iff \forall \hat{a} \equiv \tilde{a}.\ \hat{\sigma}(\hat{a}) \simD \tilde{\sigma}(\tilde{a})
  \\
  \hat{d} \simD \tilde{d} &\iff \forall \widetilde{clo} \in \tilde{d}.\ \exists \widehat{clo} \in \hat{d}.\ \widehat{clo} \simClo \widetilde{clo}
  \\
  (lam, \hat{\rho}) \simClo\ (lam, \tilde{\rho}) &\iff \hat{\rho} \simEnv \tilde{\rho}
\end{align*}
%
As thoughout, the use of $lam$ twice in the above definition indicates these components are exactly equal.


In the general case, we assume a user-provided notion of congruence for addresses produced by the standard allocator:
%
\begin{assumption}[Allocation] The allocators $\widehat{alloc}$ and $\widetilde{alloc}$ produce congruent addresses if
the input states simulate.

\label{simulation-alloc}
%
\begin{align*}
  \hat{\varsigma} \simState \tilde{\varsigma}
  \implies
  \widehat{alloc}(\vv, \hat{\varsigma}) \equiv \widetilde{alloc}(\vv, \tilde{\varsigma})
\end{align*}
%
\end{assumption}
%
In the case of both the 0-CFA and 1-CFA-style allocators we have provided, this is trivial to show as addresses are produced from a pairing of 
syntactic components which may be compared for exact equality.
%


Note that for power-set domains (e.g. $\hat{D}$) our nesting of quantification is ordered so that every element in our finite-state model must have a representative
(e.g. a closure which is at-most-as-precise) in the infinite-state model.
%
Simulation for sets of reachable configurations is inherantly one-to-many: a set of exact stacks is simulated by a single continuation-store address.
%
More precisely, a finite-state configuration $(\expr, \tilde{\rho}, \tilde{a}_\cont) \in \tilde{r}$ is simulated by the (possibly infinite) set of all pushdown states unique to the
expression $e$, and any environment $\hat{\rho}$ which simulates $\tilde{\rho}$.
%
We define this set of states using a helper $\mathcal{X}_{\hat{\xi}}(\hat{c})$ which returns an analysis result (some $\hat{\xi}_c$) representing only the partition of 
reachable states containing $\hat{c}$:
%
\begin{align*}
  \mathcal{X}_{(\hat{r},\hat{\sigma})}&((e, \hat{\rho}, \hat{\cont})) = 
        (\set{ (e, \hat{\rho}, \hat{\cont}')\ \vert\ (e, \hat{\rho}, \hat{\cont}') \in \hat{r}}, \hat{\sigma})
\end{align*}
%
We also define a transition relation $(\pdToX)$ for these partitioned, widened analyses such that:
%
\begin{align*}
  \mathcal{X}_{(\hat{r},\hat{\sigma})}&((e, \hat{\rho}, \hat{\cont})) \pdToX \mathcal{X}_{(\hat{r}',\hat{\sigma}')}((e', \hat{\rho}', \hat{\cont}')) \iff
  \\
  &(e, \hat{\rho}, \hat{\sigma}, \hat{\cont}) \pdTo (e', \hat{\rho}', \hat{\sigma}'', \hat{\cont}')\ \wedge\ (\hat{r}, \hat{\sigma}) \pdToW (\hat{r}', \hat{\sigma}')
  %%%%% Is r free or constrained to contain our (e, rho, kont) ?
\end{align*}
%
We throw away partially incremented value-stores (each $\hat{\sigma}''$) as the transition $(\pdToW)$ already defines $\hat{\sigma}'$ and it may be 
greater than the least-upper-bound of all $\hat{\sigma}''$ in any given partition.


A partition of a pushdown result simulates a single finite state when their expressions and environments simulate:
%
\begin{align*} 
  &\overbrace{\mathcal{X}_{(\hat{r},\hat{\sigma})}((e, \hat{\rho}, \hat{\cont}))}^{(\hat{r}',\hat{\sigma})} \simX (e, \tilde{\rho}, \tilde{\sigma}, \tilde{\sigma}_\cont, \tilde{a}_\cont) \iff
  \\
  \hat{\sigma} \simStore \tilde{\sigma}\ &\wedge\ \hat{\rho} \simEnv \tilde{\rho}\ \wedge\ \set{ \hat{\cont} \ \vert\ (e, \hat{\rho}, \hat{\cont}) \in \hat{r} } \simKont \tilde{a}_\cont\ \text{(via $\tilde{\sigma}_\cont$)}
\end{align*}
%
Simulation for widened finite state analyses is then defined in terms of simulation for individual finite states:
%
\begin{align*}
  &(\hat{r}, \hat{\sigma}) \simXi (\tilde{r}, \tilde{\sigma}, \tilde{\sigma}_\cont) \iff \hat{\sigma} \simStore \tilde{\sigma}\ \wedge\ 
  \\
  \forall &(e, \tilde{\rho}, \tilde{a}_\cont) \in \tilde{r}.\ \exists \hat{c} \in \hat{r}.\ \mathcal{X}_{(\hat{r}, \hat{\sigma})}(\hat{c}) \simX (e, \tilde{\rho}, \tilde{\sigma}, \tilde{\sigma}_\cont, \tilde{a}_\cont)
\end{align*}
%
Finally the heart of this connection, stack simulation, may be defined recursively.
%
The empty stack simulates the halt address in any store:
%
\begin{align*}
  \set{\epsilon} \simKont \tilde{a}_{\text{halt}} \text{  (via $\tilde{\sigma}_\cont$)} 
\end{align*}
%
Non-empty stacks simulate by the following:
%
\begin{align*}
  \hat{k} \simKont \tilde{a}_\cont \text{  (via $\tilde{\sigma}_\cont$)} \iff \tilde{a}_\cont \neq \tilde{a}_{\text{halt}}\ \wedge \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ 
  \\
  \forall((\vv, e, \tilde{\rho}), \tilde{a}_\cont') \in \tilde{\sigma}_\cont(\tilde{a}_\cont).\ \exists ((\vv, e, \hat{\rho})\!:\!\hat{\cont}) \in \hat{k}.\ \hat{\rho} \simEnv \tilde{\rho}\ \wedge\ \ \ 
  \\
  \set{ \hat{\cont}\ \vert\ ((\vv, e, \hat{\rho})\!:\!\hat{\cont}) \in \hat{k} } \simKont \tilde{a}_\cont' \text{  (via $\tilde{\sigma}_\cont$)}
\end{align*}
%



\subsection{Preliminary properties}
\label{sec:proof:lemmas}
%
We are now ready to describe some properties of this connection that make it easier to show our modeling of continuations is as precise as the unbounded-stack machine.
%
We present these without discussion as they are straightforward.
%
\begin{lemma}[Atomic-evaluation]
\label{simulation-atomic}
%
The results of atomic-evaluation simulate whenever their arguments do.
%
\begin{align*}
  \hat{\rho} \simEnv \tilde{\rho} \wedge \hat{\sigma} \simStore \tilde{\sigma}
  \implies
  \hat{\mathcal{A}}(\aexpr, \hat{\rho}, \hat{\sigma}) \simD \tilde{\mathcal{A}}(\aexpr, \tilde{\rho}, \tilde{\sigma})
\end{align*}
%
\end{lemma}
%
\begin{proof}
%
By cases on $\mathcal{A}$.
%
\end{proof}




\begin{lemma}[Flow-set-join]
\label{simulation-flowsetjoin}
%
The least-upper-bound of flow-sets will itself simulate the join of flow-sets these simulate. 
%
\begin{align*}
  \hat{d}_1 \simD \tilde{d}_1 \wedge \hat{d}_2 \simD \tilde{d}_2
  \implies
  (\hat{d}_1 \cup \hat{d}_2)  \simD  (\tilde{d}_1 \cup \tilde{d}_2)
\end{align*}
%
\end{lemma}
%
\begin{proof}
%
From the definition of $(\simD)$.
%
\end{proof}




\begin{lemma}[Store-join]
\label{simulation-storejoin}
%
The least-upper-bound of stores will itself simulate the join of the stores which these simulate. 
%
\begin{align*}
  \hat{\sigma}_1 \simStore \tilde{\sigma}_1 \wedge \hat{\sigma}_2 \simStore \tilde{\sigma}_2
  \implies
  (\hat{\sigma}_1 \join \hat{\sigma}_2)  \simStore  (\tilde{\sigma}_1 \join \tilde{\sigma}_2)
\end{align*}
%
\end{lemma}
%
\begin{proof}
%
A point-wise lifting of Lemma~\ref{simulation-flowsetjoin}.
%
\end{proof}



\begin{lemma}[Base-case]
\label{simulation-start}
%
Each abstract interpretation begins as a simulation of the other.
%
\end{lemma}
%
\begin{proof}
%
Specifically that:
%
\begin{align*}
  (\set{(e_0, \varnothing, \epsilon)}\!, \bot) \simXi (\set{(e_0, \varnothing, \tilde{a}_\text{halt})}\!, \bot, \bot)
\end{align*}
%
Falls out from the definitions given.
%
\end{proof}


\subsection{Central lemmas and theorems}
\label{sec:proof:main-theorem}
%
This section structures a proof of bisimulation between the unbounded-stack analysis and our optimized finite-state analysis.
%
We will focus exclusively on details of showing the precision of the finite-state result.
%
\begin{theorem}[Bisimulation]
%
Our abstract interpretation with a precise stack and our abstract interpretation with precise (target-state) continuation allocation precisely simulate one another.
%
\end{theorem}
%
\begin{proof}
%
By the induction argument of Lemmas \ref{simulation-start}, \ref{simulation-soundness}, and \ref{simulation-precision}.
%
\end{proof}
%
While we omit the details of the soundness half of this bisimulation proof, it directly follows from the AAM methodology \cite{might:2010:aam}.
%
\begin{lemma}[Soundness]
\label{simulation-soundness}
%
An inductive step shows that soundness is preserved across transition:
%
\begin{align*}
  \hat{\xi} \simXisound \tilde{\xi}\ \wedge\ \tilde{\xi} \fsToW \tilde{\xi}'\ \wedge\ \hat{\xi} \pdToW \hat{\xi}'
  \implies
  \hat{\xi}' \simXisound \tilde{\xi}'
\end{align*}
%
\end{lemma}

\begin{proof}
%
By cases; the reverse of Lemma~\ref{simulation-precision}.
%
\end{proof}
%
Now we come to the lemma in which we prove the precision of our analysis.
%
\begin{lemma}[Precision]
\label{simulation-precision}
%
An inductive step shows that precision is preserved across store-widened transition.
%
\begin{align*}
  \hat{\xi} \simXi \tilde{\xi}\ \wedge\ \tilde{\xi} \fsToW \tilde{\xi}'\ \wedge\ \hat{\xi} \pdToW \hat{\xi}'
  \implies
  \hat{\xi}' \simXi \tilde{\xi}'
\end{align*}
%
\end{lemma}

\begin{proof}
%
Divided into Lemmas~\ref{simulation-storeprecision} and \ref{simulation-stackprecision}.
%
\end{proof}
%
We divide this lemma into two parts. The first part shows that the precision of the globally-widened store is maintained across the transition $(\fsToW)$.
%
We omit this proof as it is very similar to the second part which more clearly focuses on the key ideas.
%
\begin{lemma}[Store-Precision]
\label{simulation-storeprecision}
%
An inductive step shows that global-store precision is preserved across transition.
%
\begin{align*}
  \hat{\xi} \simXi \tilde{\xi}\ \wedge\ \tilde{\xi} \fsToW \overbrace{(\tilde{r}', \tilde{\sigma}', \tilde{\sigma}_\cont')}^{\tilde{\xi}'}\ \wedge\ \hat{\xi} \pdToW \overbrace{(\hat{r}', \hat{\sigma}')}^{\hat{\xi}'} 
  \implies
  \hat{\sigma}' \simStore \tilde{\sigma}'
\end{align*}
%
\end{lemma}

\begin{proof}
%
Worked in a similar manner as Lemma~\ref{simulation-stackprecision}.
%
\end{proof}

Finally, we arrive at the crucial aspect of proving the precision of our optimized finite-state analysis.
%
This lemma shows that the precision of reachable configurations and stacks is maintained across the transition $(\fsToW)$.

\begin{lemma}[Reachability/Stack-Precision]
\label{simulation-stackprecision}
%
An inductive step shows that every $(\expr', \tilde{\rho}', \tilde{a}_\cont')$ reachable across a widened finite-state transition is accounted for 
by an $(\expr', \hat{\rho}', \hat{\cont}')$ reachable across a widened pushdown transition such that the partition containing $(\expr', \hat{\rho}', \hat{\cont}')$
accounts for every stack implied by $\tilde{a}_\cont'$.
%
\begin{align*}
  \hat{\xi} \simXi\ &\tilde{\xi}\ \wedge\ \overbrace{(\tilde{r}, \tilde{\sigma}, \tilde{\sigma}_\cont)}^{\tilde{\xi}} \fsToW \overbrace{(\tilde{r}', \tilde{\sigma}', \tilde{\sigma}_\cont')}^{\tilde{\xi}'}\ 
  \wedge\ \overbrace{(\hat{r}, \hat{\sigma})}^{\hat{\xi}} \pdToW \overbrace{(\hat{r}', \hat{\sigma}')}^{\hat{\xi}'} 
  \\ &\implies
  \forall (e', \tilde{\rho}', \tilde{a}_\cont') \in \tilde{r}'.\ \exists (e', \hat{\rho}', \hat{\cont}') \in \hat{r}' . \mbox{$\color{white} \simKont$} %%%%%% spacing hack %%%%%%
  \\
  &\ \ \ \ \ \ \ \ \ \ \ \ \mathcal{X}_{(\hat{r}', \hat{\sigma}')}((e', \hat{\rho}', \hat{\cont}')) \simX (e', \tilde{\rho}', \tilde{\sigma}', \tilde{\sigma}_\cont', \tilde{a}_\cont')
\end{align*}
%
\end{lemma}


\begin{proof}
%
Without loss of generality, we select a $(e', \tilde{\rho}', \tilde{a}_\cont') \in \tilde{r}'$.
%
From the antecedent $\tilde{\xi} \fsToW \tilde{\xi}'$ and the definition of $(\fsToW)$, there exist
$\tilde{\varsigma} = (e, \tilde{\rho}, \tilde{\sigma}, \tilde{\sigma}_\cont, \tilde{a}_\cont)$ and
$\tilde{\varsigma}' = (e', \tilde{\rho}', \tilde{\sigma}'', \tilde{\sigma}_\cont'', \tilde{a}_\cont')$ 
for some $\tilde{\sigma}''$ and $\tilde{\sigma}_\cont''$ such that $\tilde{\varsigma} \fsTo \tilde{\varsigma}'$.
%%%%% Say that the double-prime version are never used.
From the antecedent $\hat{\xi} \simXi \tilde{\xi}$, we know there exists a $(e, \hat{\rho}, \hat{\cont}) \in \hat{r}$ such that
$\mathcal{X}_{(\hat{r}, \hat{\sigma})}((e, \hat{\rho}, \hat{\cont})) \simX (e, \tilde{\rho}, \tilde{\sigma}, \tilde{\sigma}_\cont, \tilde{a}_\cont)$.
%
We must show that:
%
\[
	\exists (e', \hat{\rho}', \hat{\cont}') \in \hat{r}'.\ \mathcal{X}_{(\hat{r}', \hat{\sigma}')}((e', \hat{\rho}', \hat{\cont}')) \simX (e', \tilde{\rho}', \tilde{\sigma}', \tilde{\sigma}_\cont', \tilde{a}_\cont')
\]
%
For this, it is sufficient to show that:
%
\[
	\mathcal{X}_{(\hat{r}, \hat{\sigma})}((e, \hat{\rho}, \hat{\cont})) \pdToX \mathcal{X}_{(\hat{r}', \hat{\sigma}')}((e', \hat{\rho}', \hat{\cont}'))
\]
and 
\[
	\mathcal{X}_{(\hat{r}', \hat{\sigma}')}((e', \hat{\rho}', \hat{\cont}')) \simX (e', \tilde{\rho}', \tilde{\sigma}'', \tilde{\sigma}_\cont'', \tilde{a}_\cont') .
\]
%
Diagrammatically:
%
\begin{equation*}
  \begin{CD}
    \overbrace{(e, \tilde{\rho}, \tilde{\sigma}, \tilde{\sigma}_\cont, \tilde{a}_\cont)}^{\tilde{\varsigma}}  
      @> \fsTo >>  
    \overbrace{(e', \tilde{\rho}', \tilde{\sigma}'', \tilde{\sigma}_\cont'', \tilde{a}_\cont')}^{\tilde{\varsigma}'} \\
    @A \simX AA  @AA \simX A \\
    \underbrace{\mathcal{X}_{(\hat{r}, \hat{\sigma})}((e, \hat{\rho}, \hat{\cont}))}_{\hat{\xi}_c}  
      @> \pdToX >>  
    \underbrace{\mathcal{X}_{(\hat{r}', \hat{\sigma}')}((e', \hat{\rho}', \hat{\cont}'))}_{\hat{\xi}_c'} 
  \end{CD}
\end{equation*}
%
%\begin{align*}
%  \text{where}\ \ \ \ \ & (e, \tilde{\rho}, \tilde{a}_\cont) \in \tilde{r}     &(e, \hat{\rho}, \hat{\cont}) \in \hat{r}			& \ &
%                 \\
%		 & \hat{\rho} \simEnv \tilde{\rho}     &\hat{\sigma} \simStore \tilde{\sigma}			& \ &
%		 \\
%		 & K_{(e, \hat{\rho}, \_) \in \hat{r}} \simKont \tilde{a}_\cont \text{  (via $\tilde{\sigma}_\cont$)}				& \ & \ &
%\end{align*}
%
This transition $(\pdToX)$ is defined:
%
\[
	(e, \hat{\rho}, \hat{\sigma}, \hat{\cont}) \pdTo (e', \hat{\rho}', \hat{\sigma}'', \hat{\cont}')\ \wedge\ (\hat{r}, \hat{\sigma}) \pdToW (\hat{r}', \hat{\sigma}')
\]
%
The second conjunct is assumed as part of our antecedent.
%
Thus it is sufficient to show there exists a $(e', \hat{\rho}', \hat{\cont}') \in \hat{r}' $ such that $(e, \hat{\rho}, \hat{\sigma}, \hat{\cont}) \pdTo (e', \hat{\rho}', \hat{\sigma}'', \hat{\cont}')$,
for some $\hat{\sigma}''$, and
%
\[
	\mathcal{X}_{(\hat{r}', \hat{\sigma}')}((e', \hat{\rho}', \hat{\cont}')) \simX (e', \tilde{\rho}', \tilde{\sigma}'', \tilde{\sigma}_\cont'', \tilde{a}_\cont') .
\]
%
For this, we break into cases on the expression $e$.

\paragraph{[Call]} In this case our antecedent $\tilde{\varsigma} \fsTo \tilde{\varsigma}'$ expands to:
%
\begin{align*}
 \overbrace{
 (\letiform{\vv}{\appform{\fexpr}{\aexpr}}{\expr},
  \tilde{\rho},
  \tilde{\sigma},
  \tilde{\sigma}_\cont,
  \tilde{a}_\cont)}^{\tilde{\varsigma}}
 &\fsTo
 \overbrace{
 (\expr',
  \tilde{\rho}',
  \tilde{\sigma}',
  \tilde{\sigma}_\cont',
  \tilde{a}_\cont')}^{\tilde{\varsigma}'}
  \text{, where }
\end{align*}
\vspace{-0.5cm}
\begin{align*}
  (\lamform{y}{\expr'},\tilde{\rho}_\lambda) &\in
   \tilde{\mathcal{A}}(\fexpr, \tilde{\rho}, \tilde{\sigma})
  \\
  \tilde{\rho}' &= \tilde{\rho}_\lambda[y \mapsto \tilde{a}]
  \\
  \tilde{\sigma}' &= \tilde{\sigma} \join [\tilde{a} \mapsto \tilde{\mathcal{A}}(\aexpr,\tilde{\rho},\tilde{\sigma})]
  \\
  \tilde{a} &= \widetilde{alloc}(y, \tilde{\varsigma})
  \\
  \tilde{\sigma}_\cont' &= \tilde{\sigma}_\cont \join [\tilde{a}'_\cont
    \mapsto \set{ ((\vv,\expr,\tilde{\rho}),\tilde{a}_\acont) }]
  \\
  \tilde{a}'_\cont &= \widetilde{alloc}_\cont(\tilde{\varsigma}, \expr', \tilde{\rho}', \tilde{\sigma}')
\end{align*} 
%
Then the transition rule $\hat{\varsigma} \pdTo \hat{\varsigma}'$ expands to:
%
\begin{align*}
 \overbrace{
 (\letiform{x}{\appform{\fexpr}{\aexpr}}{\expr},
  \aenv,
  \astore,
  \acont)}^{\astate}
 &\pdTo
 \overbrace{
 (\expr',
  \aenv',
  \astore',
  \hat{\phi}\!:\!\acont)}^{\hat{\varsigma}'}
  \text{, where }
\end{align*}
\vspace{-0.5cm}
\begin{align*}
 \hat{\phi} &= (\vv, \expr, \aenv)
 \\
 (\lamform{y}{\expr'},\aenv_\lambda) &\in \aArgEval(\fexpr, \aenv, \astore)
 \\
 \aenv' &= \aenv_\lambda [ y \mapsto \aaddr ] 
 \\
 \astore' &= \astore \join [\aaddr \mapsto \aArgEval(\aexpr,\aenv,\astore)]
 \\
 \aaddr &= \aalloc(y,\astate)
\end{align*}
%
We fix a $(\lamform{y}{\expr'},\tilde{\rho}_\lambda) \in \tilde{\mathcal{A}}(\fexpr, \tilde{\rho}, \tilde{\sigma})$ without loss of generality.
%
Then from Lemma~\ref{simulation-atomic} we know a simulating closure exists:
%
\begin{align*}
  \exists(\lamform{y}{\expr'},\aenv_\lambda) \in \aArgEval(\fexpr, \aenv, \astore) : \hat{\rho}_\lambda \simEnv \tilde{\rho}_\lambda
\end{align*}
%
Proving our simulation decomposes into showing that:
%
\[
	\hat{\sigma}' \simStore \tilde{\sigma}'\ \wedge\ \hat{\rho}' \simEnv \tilde{\rho}'\ \wedge\ \set{ \hat{\cont}'' \ \vert\ (e', \hat{\rho}', \hat{\cont}'') \in \hat{r}' } 
	\simKont 
	\tilde{a}_\cont'\ \text{(via $\tilde{\sigma}_\cont'$)}
\]
%
Thus by Lemma~\ref{simulation-storeprecision} the first conjunct of our goal is satisfied ($\hat{\sigma}' \simStore \tilde{\sigma}'$), and by Assumption~\ref{simulation-alloc} the second conjunct of our goal is satisfied 
($\hat{\rho}' \simEnv \tilde{\rho}'$).
%
Our antecedent simulation also tells us that every stack implied by $\tilde{a}_\cont$ exists as $\hat{\cont}$ in some $\hat{\varsigma}$.
%
\begin{align*}
	\set{ \hat{\cont}'' \ \vert\ (e, \hat{\rho}, \hat{\cont}'') \in \hat{r} } 
	\simKont 
	\tilde{a}_\cont\ \text{(via $\tilde{\sigma}_\cont$)}
\end{align*}
%
From here we fix an address in the continuation-store and look at which stacks may be contributed to it across our selected $\tilde{\varsigma} \fsTo \tilde{\varsigma}'$.
%
We must ensure that every such stack is accounted for in some transition $\hat{\varsigma} \pdTo \hat{\varsigma}'$ -- and here we encounter the \textit{crucial} moment which differentiates
our technique from overly-precise AAC and previous imprecise allocation policies.


Addresses in $\tilde{a}_\cont'$, allocated across $\tilde{\varsigma} \fsTo \tilde{\varsigma}'$, are of the form $(e', \tilde{\rho}')$ and are specific to those components of our target state.
%
This means we are able to assume a $\tilde{\varsigma}$ which preceeds this expression and environment.
%
As exact stacks built across our $\hat{\varsigma} \pdTo \hat{\varsigma}'$ must always be unique to $e'$ and $\hat{\rho}'$, we may consider the cases where 
$\hat{\rho}' \simEnv \tilde{\rho}'$ and conclude that every stack implied by $\tilde{\varsigma}'$ is accounted for.
%
If instead we were to use the more common choice of $e$ or $e'$ when allocating a continuation (as is also the case for monovariant continuation-passing-style analyses),
we would need to consider transitions $\tilde{\varsigma}_{\text{other}} \fsTo \ldots$ which are not at least specific to our chosen $\tilde{\rho}'$ and show they too may only
contribute implicit stacks accounted for by our transitions to pushdown states unique to both $e'$ and $\hat{\rho}'$.
%
This is clearly not true in the general case.


%AAC on the other hand uses the entire source configuration (at least $e$ and $\tilde{\rho}$) which is at least specific to our selected $e'$ and $\tilde{\rho}'$ because predecessors determine these components of their successors uniquely.
%
%This is why AAC is as precise as our technique (and as precise as PDCFA); however, because it may be \textit{more} specific then simply $e'$ and $\tilde{\rho}'$ (various $e, \tilde{\rho}$ may preceed $e', \tilde{\rho}'$), AAC may differentiate stacks without any justifying further benefit to precision.
%
%sWe may observe here how selecting the target state is the minimal choice for obtaining perfect precision.


The continuation address we have fixed therefore is $(e', \tilde{\rho}')$ and we may also fix our contributed continuation 
$((\vv, e, \tilde{\rho}), \tilde{a}_\cont) \in \tilde{\sigma}_\cont'((e', \tilde{\rho}'))$ and demonstrate its simulation.


Without loss of generality we select the state $(e, \hat{\rho}, \hat{\cont}) \in \hat{r}$. 
%
\begin{align*}
  \exists ((\vv, e, \hat{\rho})\!:\!\hat{\cont}) \in \overbrace{\set{ \hat{\cont}'' \ \vert\ (e', \hat{\rho}', \hat{\cont}'') \in \hat{r}' }}^{\hat{k}} : \hat{\rho}' \simEnv \tilde{\rho}'\ \wedge\ \ \ \ \ \ \ \ \ \ 
  \\
  \set{ \hat{\cont}\ \vert\ ((\vv, e, \hat{\rho})\!:\!\hat{\cont}) \in \hat{k} } \simKont \tilde{a}_\cont \text{  (via $\tilde{\sigma}_\cont'$)}
\end{align*}
%
Which falls out immediately from $\hat{\varsigma} \pdTo \hat{\varsigma}'$ and our prior simulation for $\tilde{a}_\cont$.
%
This may be restated as our desired consequent:
%
\[
	\set{ \hat{\cont}'' \ \vert\ (e', \hat{\rho}', \hat{\cont}'') \in \hat{r}' } 
	\simKont 
	\tilde{a}_\cont'\ \text{(via $\tilde{\sigma}_\cont'$)}
\]
%
%
%
%
%
%


\paragraph{[Return]} In this case our antecedent $\tilde{\varsigma} \fsTo \tilde{\varsigma}'$ expands to:
%
\begin{align*}
 \overbrace{(\aexpr,
  \tilde{\rho},
  \tilde{\sigma},
  \tilde{\sigma}_\cont,
  \tilde{a}_\cont)}^{\tilde{\varsigma}}
 &\fsTo
 \overbrace{(\expr',
  \tilde{\rho}',
  \tilde{\sigma}',
  \tilde{\sigma}_\cont,
  \tilde{a}_\cont')}^{\tilde{\varsigma}'}
  \text{, where }
\end{align*}
\vspace{-0.5cm}
\begin{align*}
 ((\vv,\expr',\tilde{\rho}_\cont),\tilde{a}_\cont') &\in \tilde{\sigma}_\cont(\tilde{a}_\cont)
 \\
 \tilde{\rho}' &= \tilde{\rho}_\cont[\vv \mapsto \tilde{a}]
 \\
 \tilde{\sigma}' &= \tilde{\sigma} \join [ \tilde{a} \mapsto \tilde{\mathcal{A}}(\aexpr,\tilde{\rho},\tilde{\sigma}) ]
 \\
 \tilde{a} &= \widetilde{alloc}(\vv,\tilde{\varsigma})
\end{align*}
%
Then the transition rule $\hat{\varsigma} \pdTo \hat{\varsigma}'$ expands to:
%
\begin{align*}
 \overbrace{(\aexpr,
  \aenv,
  \astore,
  \hat{\cont})}^{\astate}
 &\pdTo
 \overbrace{
 (\expr',
  \aenv',
  \astore',
  \hat{\cont}')}^{\hat{\varsigma}'}
  \text{, where } 
\end{align*}
\vspace{-0.5cm}
\begin{align*}
 \hat{\cont} &= (\vv, \expr', \aenv_\cont)\!:\!\hat{\cont}'
 \\
 \aenv' &= \aenv_\cont[\vv \mapsto \aaddr]
 \\
 \astore' &= \astore \join [\aaddr \mapsto \aArgEval(\aexpr,\aenv,\astore)]
 \\
 \aaddr &= \aalloc(\vv,\astate)
\end{align*}
%
We unroll our simulation for $\tilde{a}_\cont$ a single step and obtain:
%
\begin{align*}
  &\overbrace{\set{ \hat{\cont}'' \ \vert\ (e', \hat{\rho}', \hat{\cont}'') \in \hat{r}' }}^{\hat{k}} \simKont \tilde{a}_\cont \text{(via $\tilde{\sigma}_\cont$)}  \implies
  \\
  \forall((\vv&, \expr', \tilde{\rho}_\cont), \tilde{a}_\cont') \in \tilde{\sigma}_\cont(\tilde{a}_\cont).\ \exists ((\vv, \expr', \hat{\rho}_\cont)\!:\!\hat{\cont}') \in \hat{k} : 
  \\
  &\hat{\rho}_\cont \simEnv \tilde{\rho}_\cont\ \wedge\ \set{ \hat{\cont}\ \vert\ ((\vv, e, \hat{\rho})\!:\!\hat{\cont}) \in \hat{k} } \simKont \tilde{a}_\cont' \text{  (via $\tilde{\sigma}_\cont$)}
\end{align*}
%
We fix $((\vv, \expr', \tilde{\rho}_\cont), \tilde{a}_\cont') \in \tilde{\sigma}_\cont(\tilde{a}_\cont)$ without loss of generality.
%
This is a specific stack frame being popped and its tail $\tilde{a}_\cont'$.
%
As our successor $\tilde{\varsigma}'$ is reached at every stack \textit{implicit} in this tail address, we must show that likewise every such stack is reached explicitly in some successor to $\hat{\varsigma}'$.


Those successors are derived from all $((\vv, \expr', \hat{\rho}_\cont)\!:\!\hat{\cont}') \in \hat{k}$.
%
We know from the existence of $\tilde{\varsigma}'$ that at least one such top frame exists.
%
We also know from $\hat{\rho}_\cont \simEnv \tilde{\rho}_\cont$ and Lemma~\ref{simulation-alloc} that $\hat{\rho}' \simEnv \tilde{\rho}'$.
%
From our unrolled simulation for $\tilde{a}_\cont$ above, we find that the total set of $\hat{\cont}'$ values transitioned to is a simulation of $\tilde{a}_\cont'$.
%
\begin{align*}
  \set{ \hat{\cont}\ \vert\ ((\vv, e', \hat{\rho}_\cont)\!:\!\hat{\cont}) \in \hat{k} } \simKont \tilde{a}_\cont'\ &\text{  (via $\tilde{\sigma}_\cont$)} \implies 
  \\
  \set{ \hat{\cont}'' \ \vert\ (e', \hat{\rho}', \hat{\cont}'') \in \hat{r}' } &\simKont \tilde{a}_\cont' \text{  (via $\tilde{\sigma}_\cont'$)}
\end{align*}



\vspace{0.4cm}
In both these cases our scheme preserves precision.
%
\end{proof}







